Optimal Stopping via Randomized Neural Networks

This paper presents the benefits of using randomized neural networks instead of standard basis functions or deep neural networks to approximate the solutions of optimal stopping problems. The key idea is to use neural networks, where the parameters of the hidden layers are generated randomly and only the last layer is trained, in order to approximate the continuation value. Our approaches are applicable to high dimensional problems where the existing approaches become increasingly impractical. In addition, since our approaches can be optimized using simple linear regression, they are easy to implement and theoretical guarantees can be provided. We test our approaches for American option pricing on Black--Scholes, Heston and rough Heston models and for optimally stopping a fractional Brownian motion. In all cases, our algorithms outperform the state-of-the-art and other relevant machine learning approaches in terms of computation time while achieving comparable results. Moreover, we show that they can also be used to efficiently compute Greeks of American options.

==> tables/table_Dim_RoughHeston_MaxCallr0_gt1.tex <==

\begin{table*}[!h]
\center
\scalebox{0.480}{
\begin{tabular}{|cc|r r r r r r r r|r r r r r r r r|}
\toprule
    & {} & \multicolumn{8}{c |}{price} & \multicolumn{8}{c |}{duration} \\
$d$ & use P & LSM & DOS & pathDOS & NLSM & RLSM & RRLSM & FQI & RFQI & LSM & DOS & pathDOS & NLSM & RLSM & RRLSM & FQI & RFQI\\
\midrule
\multirow{2}{*}{5} & False &   8.60 (0.07) &   7.29 (0.08) &   7.11 (0.07) &   8.71 (0.11) &   8.51 (0.08) &   8.61 (0.08) &   8.26 (0.07) &   7.99 (0.23) &        9s &       9s &        9s &       3s &       0s &       0s &        2s &       0s \\
    & True  &   8.83 (0.05) &   8.77 (0.07) &   8.77 (0.08) &   8.64 (0.09) &   8.73 (0.13) &   8.73 (0.08) &   2.24 (0.25) &   6.85 (0.85) &       11s &       7s &       10s &       3s &       0s &       0s &        3s &       0s \\
\cline{1-18}
\multirow{2}{*}{10} & False &  12.92 (0.11) &  10.39 (0.05) &  10.32 (0.06) &  12.92 (0.09) &  12.90 (0.09) &  12.96 (0.11) &  12.32 (0.11) &  10.76 (0.43) &       23s &       7s &       13s &       3s &       0s &       0s &        8s &       0s \\
    & True  &  13.14 (0.08) &  12.98 (0.11) &  12.98 (0.06) &  12.93 (0.05) &  13.07 (0.13) &  12.70 (0.16) &   8.27 (1.95) &  11.14 (0.24) &       27s &       7s &       14s &       3s &       0s &       0s &       11s &       0s \\
\cline{1-18}
\multirow{2}{*}{50} & False &  25.50 (0.14) &  19.86 (0.15) &  20.24 (0.12) &  26.04 (0.11) &  26.00 (0.13) &  25.98 (0.09) &  22.90 (0.53) &  17.29 (0.16) &     7m57s &       8s &       52s &       3s &       0s &       0s &     7m 8s &       1s \\
    & True  &  24.67 (0.14) &  25.95 (0.17) &  25.75 (0.11) &  26.02 (0.14) &  25.78 (0.14) &  25.78 (0.16) &  26.00 (0.23) &  21.55 (0.71) &     8m 8s &       8s &       57s &       3s &       0s &       0s &     7m17s &       1s \\
\cline{1-18}
\multirow{2}{*}{100} & False &  29.48 (0.12) &  25.21 (0.22) &  27.60 (0.17) &  32.37 (0.13) &  32.82 (0.09) &  32.75 (0.10) &  29.05 (1.99) &  24.55 (0.19) &    38m 9s &      10s &     1m21s &       4s &       0s &       0s &  1h23m 7s &       1s \\
    & True  &  28.50 (0.12) &  32.79 (0.13) &  32.30 (0.14) &  32.37 (0.28) &  32.57 (0.15) &  32.64 (0.16) &  28.97 (2.32) &  27.59 (0.50) &    39m17s &       9s &     1m24s &       4s &       0s &       0s &  1h26m47s &       1s \\
\bottomrule
\end{tabular}

}
\caption{Max call option on Rough--Heston for different number of stocks $d$. The interest rate is $r=5\%$ and the dividend rate is $\delta = 10\%$.
}
\label{table_Dim_RoughHeston_MaxCallr0_gt1}
\end{table*}


==> tables/table_GeoPut_HestonV_payoffs_gt1.tex <==

\begin{table*}[!h]
\center
\scalebox{0.60}{
\begin{tabular}{|cc|r r r r r r|r r r r r r|}
\toprule
   & {} & \multicolumn{6}{c |}{price} & \multicolumn{6}{c |}{duration} \\
$d$ & use P & LSM & DOS & NLSM & RLSM & FQI & RFQI & LSM & DOS & NLSM & RLSM & FQI & RFQI\\
\midrule
\multirow{2}{*}{1} & False &  4.16 (0.05) &  4.15 (0.07) &  4.07 (0.06) &  4.10 (0.08) &  4.13 (0.06) &  4.13 (0.05) &        3s &       5s &       1s &       0s &        1s &       0s \\
   & True  &  4.15 (0.06) &  4.14 (0.05) &  4.11 (0.08) &  4.15 (0.05) &  4.14 (0.08) &  4.15 (0.03) &        5s &       5s &       1s &       0s &        1s &       0s \\
\cline{1-14}
\multirow{2}{*}{5} & False &  2.40 (0.02) &  2.45 (0.03) &  2.33 (0.04) &  2.39 (0.03) &  2.46 (0.03) &  2.43 (0.03) &       24s &       5s &       1s &       0s &        8s &       0s \\
   & True  &  2.41 (0.03) &  2.43 (0.03) &  2.35 (0.05) &  2.44 (0.02) &  2.45 (0.03) &  2.45 (0.03) &       28s &       5s &       1s &       0s &        9s &       0s \\
\cline{1-14}
\multirow{2}{*}{10} & False &  1.93 (0.02) &  1.99 (0.02) &  1.75 (0.04) &  1.97 (0.03) &  2.02 (0.02) &  1.96 (0.16) &     1m23s &       6s &       2s &       0s &       33s &       0s \\
   & True  &  1.93 (0.02) &  1.99 (0.02) &  1.77 (0.05) &  2.01 (0.03) &  2.02 (0.02) &  2.01 (0.02) &     1m31s &       6s &       1s &       0s &       37s &       0s \\
\cline{1-14}
\multirow{2}{*}{20} & False &  1.53 (0.02) &  1.68 (0.02) &  1.27 (0.04) &  1.62 (0.05) &  1.71 (0.02) &  1.69 (0.09) &     5m21s &       6s &       2s &       0s &     3m22s &       1s \\
   & True  &  1.53 (0.02) &  1.69 (0.02) &  1.27 (0.03) &  1.63 (0.07) &  1.71 (0.02) &  1.60 (0.30) &     5m35s &       6s &       2s &       0s &     3m39s &       1s \\
\bottomrule
\end{tabular}

}
\caption{Algorithms were run $10$ times and the mean and the standard deviation (in parenthesis) of the prices as well as the median of the computation time are given.. model = HestonWithVar, payoff = GeometricPut, drift = 0.02, $x_0$ = 100, volatility = 0.2, nb\_paths = 20000, nb\_dates = 10, strike = 100, dividend = 0.0, maturity = 1, hidden\_size = 20, nb\_epochs = 30, hurst = 0.75, factors = (1.0, 1.0, 1.0), ridge\_coeff = 1.0, use\_path = False, train\_ITM\_only = True.
}
\label{table_GeoPut_HestonV_payoffs_gt1}
\end{table*}


==> tables/table_GeoPut_payoffsr0_gt.tex <==

\begin{table*}[!h]
\center
\scalebox{0.61}{
\begin{tabular}{|cc|r r r r r r|r r r r r r|}
\toprule
       & {} & \multicolumn{6}{c |}{price} & \multicolumn{6}{c |}{duration} \\
model & $d$ & LSM & DOS & NLSM & RLSM & FQI & RFQI & LSM & DOS & NLSM & RLSM & FQI & RFQI\\
\midrule
\multirow{4}{*}{BlackScholes} & 1  &  7.10 (0.09) &  6.98 (0.10) &  7.06 (0.11) &  7.07 (0.09) &  6.93 (0.10) &  6.95 (0.08) &        2s &       6s &       1s &       0s &       0s &       0s \\
       & 5  &  3.34 (0.05) &  3.35 (0.06) &  3.31 (0.05) &  3.30 (0.02) &  3.31 (0.05) &  3.35 (0.04) &        9s &       5s &       1s &       0s &       2s &       0s \\
       & 10 &  2.37 (0.03) &  2.37 (0.03) &  2.37 (0.03) &  2.36 (0.03) &  2.39 (0.03) &  2.40 (0.03) &       24s &       6s &       1s &       0s &       7s &       0s \\
       & 20 &  1.67 (0.01) &  1.67 (0.03) &  1.59 (0.05) &  1.64 (0.03) &  1.73 (0.04) &  1.72 (0.02) &     1m23s &       6s &       1s &       0s &      32s &       1s \\
\cline{1-14}
\multirow{4}{*}{Heston} & 1  &  4.13 (0.07) &  4.09 (0.07) &  4.13 (0.07) &  4.11 (0.04) &  4.17 (0.06) &  4.15 (0.08) &        2s &       5s &       1s &       0s &       0s &       0s \\
       & 5  &  2.43 (0.02) &  2.42 (0.03) &  2.30 (0.05) &  2.40 (0.03) &  2.44 (0.04) &  2.43 (0.03) &        9s &       6s &       1s &       0s &       2s &       0s \\
       & 10 &  2.00 (0.02) &  2.00 (0.02) &  1.77 (0.08) &  1.98 (0.02) &  2.00 (0.02) &  2.01 (0.02) &       24s &       6s &       2s &       0s &       7s &       0s \\
       & 20 &  1.68 (0.01) &  1.70 (0.02) &  1.21 (0.04) &  1.60 (0.07) &  1.72 (0.02) &  1.71 (0.01) &     1m23s &       7s &       2s &       0s &      32s &       1s \\
\bottomrule
\end{tabular}

}
\caption{Geometric put options on Black--Scholes and Heston for different number of stocks $d$. Here $r = 2\%$ is used for the drift. \OurAlgoRS achieves the highest prices while being the fastest and having considerably less trainable parameters. 
}
\label{table_GeoPut_payoffsr0_gt}
\end{table*}


==> tables/table_GeoPut_payoffsr0_gt1.tex <==

\begin{table*}[!h]
\center
\scalebox{0.58}{
\begin{tabular}{|ccc|r r r r r r|r r r r r r|}
\toprule
       &    & {} & \multicolumn{6}{c |}{price} & \multicolumn{6}{c |}{duration} \\
model & $d$ & use P & LSM & DOS & NLSM & RLSM & FQI & RFQI & LSM & DOS & NLSM & RLSM & FQI & RFQI\\
\midrule
\multirow{8}{*}{BlackScholes} & \multirow{2}{*}{1} & False &  7.10 (0.09) &  6.98 (0.10) &  7.06 (0.11) &  7.07 (0.09) &  6.93 (0.10) &  6.95 (0.08) &        2s &       6s &       1s &       0s &       0s &       0s \\
       &    & True  &  7.04 (0.12) &  7.10 (0.05) &  7.08 (0.07) &  7.05 (0.09) &  6.98 (0.09) &  6.99 (0.35) &        3s &       5s &       1s &       0s &       0s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{5} & False &  3.34 (0.05) &  3.35 (0.06) &  3.31 (0.05) &  3.30 (0.02) &  3.31 (0.05) &  3.35 (0.04) &        9s &       5s &       1s &       0s &       2s &       0s \\
       &    & True  &  3.34 (0.04) &  3.31 (0.03) &  3.29 (0.06) &  3.33 (0.04) &  3.33 (0.03) &  3.34 (0.04) &       11s &       6s &       1s &       0s &       3s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{10} & False &  2.37 (0.03) &  2.37 (0.03) &  2.37 (0.03) &  2.36 (0.03) &  2.39 (0.03) &  2.40 (0.03) &       24s &       6s &       1s &       0s &       7s &       0s \\
       &    & True  &  2.37 (0.04) &  2.42 (0.02) &  2.33 (0.02) &  2.40 (0.04) &  2.39 (0.03) &  2.39 (0.03) &       28s &       6s &       1s &       0s &       9s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{20} & False &  1.67 (0.01) &  1.67 (0.03) &  1.59 (0.05) &  1.64 (0.03) &  1.73 (0.04) &  1.72 (0.02) &     1m23s &       6s &       1s &       0s &      32s &       1s \\
       &    & True  &  1.65 (0.02) &  1.71 (0.04) &  1.57 (0.04) &  1.65 (0.03) &  1.72 (0.03) &  1.70 (0.02) &     1m31s &       6s &       1s &       0s &      36s &       1s \\
\cline{1-15}
\cline{2-15}
\multirow{8}{*}{Heston} & \multirow{2}{*}{1} & False &  4.13 (0.07) &  4.09 (0.07) &  4.13 (0.07) &  4.11 (0.04) &  4.17 (0.06) &  4.15 (0.08) &        2s &       5s &       1s &       0s &       0s &       0s \\
       &    & True  &  4.16 (0.08) &  4.10 (0.06) &  4.10 (0.08) &  4.11 (0.07) &  4.18 (0.06) &  3.86 (0.55) &        3s &       5s &       2s &       0s &       1s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{5} & False &  2.43 (0.02) &  2.42 (0.03) &  2.30 (0.05) &  2.40 (0.03) &  2.44 (0.04) &  2.43 (0.03) &        9s &       6s &       1s &       0s &       2s &       0s \\
       &    & True  &  2.45 (0.03) &  2.44 (0.03) &  2.30 (0.06) &  2.44 (0.02) &  2.46 (0.02) &  2.45 (0.03) &       11s &       6s &       1s &       0s &       3s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{10} & False &  2.00 (0.02) &  2.00 (0.02) &  1.77 (0.08) &  1.98 (0.02) &  2.00 (0.02) &  2.01 (0.02) &       24s &       6s &       2s &       0s &       7s &       0s \\
       &    & True  &  2.00 (0.02) &  2.00 (0.02) &  1.75 (0.04) &  2.00 (0.03) &  2.01 (0.03) &  2.00 (0.02) &       29s &       6s &       2s &       0s &       9s &       0s \\
\cline{2-15}
       & \multirow{2}{*}{20} & False &  1.68 (0.01) &  1.70 (0.02) &  1.21 (0.04) &  1.60 (0.07) &  1.72 (0.02) &  1.71 (0.01) &     1m23s &       7s &       2s &       0s &      32s &       1s \\
       &    & True  &  1.68 (0.02) &  1.69 (0.02) &  1.21 (0.05) &  1.62 (0.05) &  1.71 (0.02) &  1.72 (0.02) &     1m31s &       7s &       2s &       0s &      35s &       1s \\
\bottomrule
\end{tabular}

}
\caption{Geometric put options on Black--Scholes and Heston for different number of stocks $d$. Here $r = 2\%$ is used for the drift. \OurAlgoRS achieves the highest prices while being the fastest and having considerably less trainable parameters.
}
\label{table_GeoPut_payoffsr0_gt1}
\end{table*}


==> tables/table_spots_Dim_HestonV_MinPut_gt.tex <==

\begin{table*}[!h]
\center
\scalebox{0.60}{
\begin{tabular}{|c|r r r r r r|r r r r r r|}
\toprule
{} & \multicolumn{6}{c |}{price} & \multicolumn{6}{c |}{duration} \\
$d$ & LSM & DOS & NLSM & RLSM & FQI & RFQI & LSM & DOS & NLSM & RLSM & FQI & RFQI\\
\midrule
5         &  12.34 (0.05) &  12.31 (0.05) &  12.16 (0.11) &  12.29 (0.06) &  12.40 (0.08) &  12.39 (0.11) &       30s &        6s &        3s &       0s &        9s &       0s \\
10        &  16.48 (0.07) &  16.52 (0.08) &  16.09 (0.13) &  16.55 (0.06) &  16.61 (0.04) &  16.63 (0.11) &     1m31s &        6s &        3s &       0s &       29s &       0s \\
50        &  22.86 (0.05) &  25.56 (0.04) &  24.03 (0.42) &  24.85 (0.08) &  25.69 (0.07) &  25.73 (0.03) &    39m57s &        9s &        4s &       0s &  1h26m57s &       1s \\
100       &             - &  29.13 (0.04) &  27.30 (0.46) &  28.50 (0.06) &             - &  29.36 (0.08) &         - &       16s &        6s &       0s &         - &       1s \\
500       &             - &  36.26 (0.05) &  34.74 (0.31) &  36.28 (0.04) &             - &  36.96 (0.06) &         - &     1m21s &       24s &       3s &         - &       2s \\
1000      &             - &  38.62 (0.08) &  38.19 (0.20) &  39.32 (0.03) &             - &  39.97 (0.04) &         - &     3m18s &       45s &       6s &         - &       4s \\
2000      &             - &  39.22 (0.13) &  41.05 (0.21) &  42.22 (0.04) &             - &  42.82 (0.03) &         - &    12m51s &     1m37s &      13s &         - &       8s \\
\bottomrule
\end{tabular}

}
\caption{Min put option on Heston (with variance) for different number of stocks $d$ and varying initial stock price $x_0$. Here $r=2\%$ is used as rate. The payoff is used as additional input.
}
\label{table_$x_0$s_Dim_HestonV_MinPut_gt}
\end{table*}

